Gate modulation of the hole singlet-triplet qubit frequency in germanium

Spin qubits in germanium gate-defined quantum dots have made considerable progress within the last few years, partially due to their strong spin-orbit coupling and site-dependent $g$-tensors. While this characteristic of the $g$-factors removes the need for micromagnets and allows for the possibility of all-electric qubit control, relying on these $g$-tensors necessitates the need to understand their sensitivity to the confinement potential that defines the quantum dots. Here, we demonstrate a $S-T\_$ qubit whose frequency is a strong function of the voltage applied to the barrier gate shared by the quantum dots. We find a $g$-factor that can be approximately increased by an order of magnitude adjusting the barrier gate voltage only by 12 mV. We attribute the strong dependence to a variable strain profile in our device. This work not only reinforces previous findings that site-dependent $g$-tensors in germanium can be utilized for qubit manipulation, but reveals the sensitivity and tunability these $g$-tensors have to the electrostatic confinement of the quantum dot.

==> latexmkrc <==
$sub_doc_output = 'output-subdoc';

@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {

             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
